Dijet production in diffractive deep inelastic scattering at HERA

The production of dijets in diffractive deep inelastic scattering has been measured with the ZEUS detector at HERA using an integrated luminosity of $61 \pbi$. The dijet cross section has been measured for virtualities of the exchanged virtual photon, $5 < Q^2 < 100 \gev^2$, and $\gamma^{*} p$ centre-of-mass energies, 100 < W < 250 GeV. The jets, identified using the inclusive k_{T} algorithm in the $\gamma^* p$ frame, were required to have a transverse energy $E^*_{T, \rm jet} > 4 \gev$ and the jet with the highest transverse energy was required to have $E^*_{T,\rm jet} > 5 \gev$. All jets were required to be in the pseudorapidity range $-3.5 < \eta^*_{\rm jet} < 0$. The differential cross sections are compared to leading-order predictions and next-to-leading-order QCD calculations based on recent diffractive parton densities extracted from inclusive diffractive deep inelastic scattering data.

==> DESY-07-126-cit.tex <==
%==============================================================================
%	Some definitions of citations
%==============================================================================

%------------------------------------------------------------------------------
%	-> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
%	-> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}


==> DESY-07-126-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{./BiBTeX/user/syn.bib,%
              ./BiBTeX/bib/l4z_articles.bib,%
              ./BiBTeX/bib/l4z_books.bib,%
              ./BiBTeX/bib/l4z_conferences.bib,%
              ./BiBTeX/bib/l4z_h1.bib,%
              ./BiBTeX/bib/l4z_misc.bib,%
              ./BiBTeX/bib/l4z_old.bib,%
              ./BiBTeX/bib/l4z_preprints.bib,%
              ./BiBTeX/bib/l4z_replaced.bib,%
              ./BiBTeX/bib/l4z_temporary.bib,%
              ./BiBTeX/bib/l4z_zeus.bib}}
}
\vfill\eject

